Kolmogorov-Arnold causal generative models

Causal generative models provide a principled framework for answering observational, interventional, and counterfactual queries from observational data. However, many deep causal models rely on highly expressive architectures with opaque mechanisms, limiting auditability in high-stakes domains. We propose KaCGM, a causal generative model for mixed-type tabular data where each structural equation is parameterized by a Kolmogorov--Arnold Network (KAN). This decomposition enables direct inspection of learned causal mechanisms, including symbolic approximations and visualization of parent--child relationships, while preserving query-agnostic generative semantics. We introduce a validation pipeline based on distributional matching and independence diagnostics of inferred exogenous variables, allowing assessment using observational data alone. Experiments on synthetic and semi-synthetic benchmarks show competitive performance against state-of-the-art methods. A real-world cardiovascular case study further demonstrates the extraction of simplified structural equations and interpretable causal effects. These results suggest that expressive causal generative modeling and functional transparency can be achieved jointly, supporting trustworthy deployment in tabular decision-making settings. Code: https://github.com/aalmodovares/kacgm

==> math_commands.tex <==
\RequirePackage{mathtools}
\RequirePackage{amsmath,amsfonts,bm}
\RequirePackage{suffix}

% punctuation of equations, see for example the first answer in
% https://www.reddit.com/r/LaTeX/comments/5xnzg7/correct_grammar_for_putting_an_equation/
\newcommand{\equationPunctuation}[1]{\,{#1}}

%% Bold greek letters
\newcommand{\thetab}{{\boldsymbol{\theta}}}
\newcommand{\betab}{{\boldsymbol{\beta}}}
\newcommand{\pib}{{\boldsymbol{\pi}}}
\newcommand{\taub}{{\boldsymbol{\tau}}}
\newcommand{\psib}{{\boldsymbol{\psi}}}
\newcommand{\phib}{{\boldsymbol{\phi}}}
\newcommand{\omegab}{{\boldsymbol{\omega}}}
\newcommand{\etab}{{\boldsymbol{\eta}}}
\newcommand{\sigmab}{{\boldsymbol{\sigma}}}
\newcommand{\epsilonb}{{\boldsymbol{\epsilon}}}

\newcommand{\Thetab}{{\boldsymbol{\Theta}}}

\newcommand{\distribution}[1][]{\ensuremath{{P}_{#1}}\xspace}
\newcommand{\cumulative}[1][]{\ensuremath{F_{#1}}\xspace}
\newcommand{\empcumulative}[1][]{\ensuremath{\hat F_{#1}}\xspace}
\newcommand{\pushforward}[2]{{#1}_{\#} {#2}}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclarePairedDelimiter{\Ebrackets}{[}{]}
\newcommand{\Expect}[2][]{\E_{#1}\Ebrackets{#2}}
\WithSuffix\newcommand\Expect*[2][]{\E_{#1}\Ebrackets*{#2}}

\DeclareMathOperator{\V}{\mathbb{V}}
\newcommand{\Var}[2][]{\V_{#1}\Ebrackets{#2}}

\newcommand{\normal}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\uniform}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\categorical}{\ensuremath{\operatorname{Cat}}\xspace}
\newcommand{\bernoulli}{\ensuremath{\operatorname{Bern}}\xspace}
\newcommand{\binomial}{\ensuremath{\operatorname{Bin}}\xspace}
\newcommand{\lognormal}{\ensuremath{\operatorname{Log-normal}}\xspace}
\newcommand{\poisson}{\ensuremath{\operatorname{Poiss}}\xspace}
\newcommand{\exponentialdistribution}{\ensuremath{\operatorname{Exp}}\xspace}
\newcommand{\betadistribution}{\ensuremath{\operatorname{Beta}}\xspace}
\newcommand{\weibulldistribution}{\ensuremath{\operatorname{Weibull}}\xspace}

\newcommand{\identity}{\ensuremath{\mI}}
\newcommand{\indicator}[1]{\ensuremath{\mathbf{1}_{\{#1\}}}}
\newcommand{\ones}{\ensuremath{\mathbf{1}}\xspace}
\newcommand{\zeroes}{\ensuremath{\mathbf{0}}\xspace}

\DeclareMathOperator*{\avg}{avg}
\DeclareMathOperator*{\med}{med}
\DeclareMathOperator*{\std}{std}

\let\cossim\cos

%%%%%%

\usepackage{suffix}
\usepackage{xparse}
\usepackage{mathtools}

%%%%
\def\rL{{\textnormal{L}}}
\def\rvL{{\mathbf{L}}}
\def\ervL{{\textnormal{L}}}

\def\rM{{\textnormal{M}}}
\def\rvM{{\mathbf{M}}}
\def\ervM{{\textnormal{M}}}

\def\vT{\bm{T}}
\def\vF{\bm{F}}
\def\vR{\bm{R}}
\def\vU{\bm{U}}
\def\rU{{\textnormal{U}}}
\def\rvU{{\mathbf{U}}}
\def\ervU{{\textnormal{U}}}
%%%%

\newcommand{\tensor}[1]{\ensuremath{\mathsf{#1}}}
\renewcommand{\vec}{\operatorname{vec}}
\newcommand{\D}{\mathrm{D}}
\newcommand{\Gmat}{\mathrm{G}}
\newcommand{\F}{\mathrm{F}}
\newcommand{\He}{\mathrm{H}}
\newcommand{\HeCal}{\mathcal{H}}
%\newcommand{\diff}{\mathrm{d}}
\newcommand*\dif{\mathop{}\!\mathrm{d}}
\newcommand{\average}[1]{\overline{ #1 }}

\newcommand{\Loss}{\mathcal{L}}
\newcommand{\jac}{\mathrm{J}}
\newcommand{\lin}[1]{\left\langle #1 \right\rangle}

\newcommand{\nablasquaredsub}[1]{
  \nabla^{\kern -.0em \raise.1em\hbox{\tiny$2$}} {\kern -.6em \raise-.1em\hbox{\tiny$#1$}}{}
}
\newcommand{\nablasub}[1]{
  \nabla {\kern -.2em \raise-.1em\hbox{\tiny$#1$}}{}
}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\bfseries \color{maincolor} (a)}\xspace}
\newcommand{\captionb}{{\bfseries \color{maincolor}  (b)}\xspace}
\newcommand{\captionc}{{\bfseries \color{maincolor}  (c)}\xspace}
\newcommand{\captiond}{{\bfseries \color{maincolor}  (d)}\xspace}


% Added by me (@Adrian) to be consinstent when I do listings
\newcommand{\itemi}{{\bfseries \color{maincolor} i)}\xspace}
\newcommand{\itemii}{{\bfseries \color{maincolor} ii)}\xspace}
\newcommand{\itemiii}{{\bfseries \color{maincolor} iii)}\xspace}
\newcommand{\itemiv}{{\bfseries \color{maincolor} iv)}\xspace}
\newcommand{\itemv}{{\bfseries \color{maincolor} v)}\xspace}
\newcommand{\itemvi}{{\bfseries \color{maincolor} vi)}\xspace}
\newcommand{\itemvii}{{\bfseries \color{maincolor} vii)}\xspace}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvi{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vnu{{\bm{\nu}}}
\def\vtheta{{\bm{\theta}}}
\def\vgamma{{\bm{\gamma}}}
\def\vdelta{{\bm{\delta}}}
\def\vDelta{{\bm{\Delta}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vehat{\bm{\hat{e}}}
\def\vetilde{\bm{\tilde{e}}}
\def\vell{{\bm{\ell}}}
\def\vf{{\bm{f}}}
\def\vfhat{{\bm{\hat{f}}}}
\def\vg{{\bm{g}}}
\def\vgtilde{\bm{\tilde{g}}}
\def\vghat{\bm{\hat{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vmhat{{\bm{\hat{m}}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vphi{{\bm{\phi}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vstilde{\bm{\tilde{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vvhat{{\bm{\hat{v}}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vytilde{{\bm{\tilde{y}}}}
\def\vyhat{{\bm{\hat{y}}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evyhat{{\hat{y}}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mGtilde{\bm{\tilde{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mWhat{{\bm{\hat{W}}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mPi{{\bm{\Pi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}
\def\mStilde{\bm{\tilde{\mS}}}
\def\mGtilde{\bm{\tilde{\mG}}}
\def\mGoverline{{\bm{\overline{G}}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sYhat{{\hat{\mathbb{Y}}}}
\def\sZ{{\mathbb{Z}}}
% Blackboard Greek characters: https://tex.stackexchange.com/a/3260
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\def\sOmega{{\mathbbold{\Omega}}}
\def\sPhi{{\mathbbold{\Phi}}}
\def\sTheta{{\mathbbold{\Theta}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}
\def\emPi{{\Pi}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdf}{\ensuremath{p}\xspace}
\newcommand{\cdf}{\ensuremath{F}\xspace}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\mathrm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\mathrm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\mathrm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\ifcsname laplace\endcsname%
    \renewcommand{\laplace}{\mathrm{Laplace}}% Laplace distribution
\else%
    \newcommand{\laplace}{\mathrm{Laplace}}% Laplace distribution
\fi

%\newcommand{\E}{\mathbb{E}}
%\DeclareMathOperator{\E}{\mathbb{E}}

\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\onehot}{\mathrm{onehot}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
%\newcommand{\KL}{D_{\mathrm{KL}}}
%\DeclareMathOperator{\KL}{KL}
%\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

%\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \newcommand{\parents}[1]{{\ensuremath{\mathrm{pa}_{#1}}\xspace}}
% \newcommand{\ancestors}[1]{{\ensuremath{\mathrm{an}_{#1}}\xspace}}
% \newcommand{\children}[1]{{\ensuremath{\mathrm{ch}_{#1}}\xspace}}

\newcommand{\parents}[1]{{\ensuremath{\mathrm{pa}(#1)}\xspace}}
\newcommand{\ancestors}[1]{{\ensuremath{\mathrm{an}(#1)}\xspace}}
\newcommand{\children}[1]{{\ensuremath{\mathrm{ch}(#1)}\xspace}}
\newcommand{\descendants}[1]{{\ensuremath{\mathrm{de}(#1)}\xspace}}

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\minimize}{minimize}
%\DeclareMathOperator*{\maximize}{maximize}

\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\mean}{mean}
\DeclareMathOperator{\vmap}{vmap}
\DeclareMathOperator{\reshape}{reshape}
%\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\eig}{eig}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\vecspan}{span}
\DeclareMathOperator{\overlap}{overlap}
\DeclareMathOperator{\Cat}{Cat}

%%%%% NEW MATH DEFINITIONS %%%%%
\newcommand{\grad}[1]{\ensuremath{\nabla_{\!{#1}}}}
\newcommand{\naturalgrad}[1]{\ensuremath{\tilde{\nabla}_{\!{#1}}}}
\newcommand{\gradsquared}[1]{\ensuremath{\nabla_{\!{#1}}^{2}}}
\newcommand{\hess}[1]{\ensuremath{\mathrm{H}_{#1}}}

\newcommand{\Dtrain}{\ensuremath{\sD_{\mathrm{train}}}}
\newcommand{\Dtest}{\ensuremath{\sD_{\mathrm{test}}}}
\newcommand{\Dvalid}{\ensuremath{\sD_{\mathrm{valid}}}}


% || for KLDivergence
\DeclarePairedDelimiterX{\KLdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\KLdiv}{\KL\KLdivx}

\NewDocumentCommand{\giventhat}{O{\;|} m m}{#2#1\;#3}

\let\ab\allowbreak


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End:


==> my_commands.tex <==

%%% Colors
\colorlet{idcolor}{greendark}
\colorlet{unidcolor}{SBred}
\colorlet{hiddencolor}{gray}

\newcommand{\maincolor}{\textcolor{maincolor}{blue}\xspace}
\newcommand{\Maincolor}{\textcolor{maincolor}{Blue}\xspace}
\let\firstcolor\maincolor
\let\Firstcolor\Maincolor
\newcommand{\secondcolor}{\textcolor{secondcolor}{red}\xspace}
\newcommand{\Secondcolor}{\textcolor{secondcolor}{Red}\xspace}

%%% Boxes

\newtcolorbox{takeaway}{
    colback=maincolor!5!white, colframe=maincolor!75!black
}

%%% Text

\newcommand{\methodname}[1]{\texttt{\small #1}}


%%%
\newcommand{\ours}{{KaCGM}\xspace} % TODO change
\newcommand{\Ours}{{KaCGM}\xspace}
\newcommand{\ourslong}{Kolmogorov-Arnold causal generative model\xspace}
\newcommand{\oursmix}{{$\text{\ours}_\text{mix}$}\xspace}


\newcommand{\eqcomment}[1]{\text{[\textit{#1}]}}

%%% SYMBOLS

\newcommand{\kanlayer}{\ensuremath{\phi}\xspace}
\newcommand{\kanoutlayer}{\ensuremath{\Phi}\xspace}
\newcommand{\kan}{\ensuremath{\boldsymbol\Phi}\xspace}
\newcommand{\loss}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\ELBO}{\ensuremath{\mathcal{L}_\text{ELBO}}\xspace}
\newcommand{\regularization}{\ensuremath{\mathcal{R}}\xspace}

\newcommand{\parameters}{\ensuremath{\theta}\xspace}
\newcommand{\parametersq}{\ensuremath{\phi}\xspace}
\newcommand{\parametersqq}{\ensuremath{\psi}\xspace}

%\let\pred\tilde
\renewcommand{\cond}[1]{{|{#1}}}
\newcommand{\pred}[1]{\ensuremath{\tilde{#1}}\xspace}
\newcommand{\factual}[1]{\ensuremath{{#1}^\text{\normalfont{f}}}}
\newcommand{\cfactual}[1]{\ensuremath{{#1}^\text{\normalfont{cf}}}}

\newcommand{\indexone}{\ensuremath{i}\xspace}
\newcommand{\indextwo}{\ensuremath{j}\xspace}
\newcommand{\indexthree}{\ensuremath{k}\xspace}
\newcommand{\indexfour}{\ensuremath{q}\xspace}
\newcommand{\indexlayer}{\ensuremath{l}\xspace}
\newcommand{\indexfive}{\ensuremath{r}\xspace}
\newcommand{\indexsix}{\ensuremath{s}\xspace}

\newcommand{\indexcovariate}{\indextwo}
\newcommand{\indexsample}{\indexone}

\newcommand{\nLayers}{\ensuremath{L}\xspace}

\newcommand{\query}{\ensuremath{Q}\xspace}

\newcommand{\doop}{\text{do}}
\newcommand{\intervention}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\sampleintervention}{\ensuremath{\alpha}\xspace}
\newcommand{\indexintervention}{\ensuremath{\indexone}\xspace}

\newcommand{\scmfamily}{\ensuremath{\mathbb{M}}\xspace}
\newcommand{\scm}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\gcm}{\ensuremath{\pred{\scm}}\xspace}
\newcommand{\graph}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\func}[1][]{\ensuremath{f_{#1}}\xspace}
\newcommand{\funcb}[1][]{\ensuremath{\mathbf{f}_{#1}}\xspace}
\newcommand{\predfuncb}[1][]{\ensuremath{{\pred{\mathbf{f}}}_{#1}}\xspace}
\newcommand{\funcg}[1][]{\ensuremath{g_{#1}}\xspace}
\newcommand{\funcbg}[1][]{\ensuremath{\mathbf{g}_{#1}}\xspace}
\newcommand{\predfuncg}[1][]{\ensuremath{{\pred{\mathbf{f}}}_{#1}}\xspace}

\newcommand{\varparents}[2][\varobs]{\ensuremath{\parents{#2}}\xspace}
\newcommand{\varchildren}[2][\varobs]{\ensuremath{\children{#2}}\xspace}

\newcommand{\edist}{\ensuremath{\tilde{p}}\xspace}

\newcommand{\dataset}{\ensuremath{\gD}\xspace}

\newcommand{\outcome}{\ensuremath{\rvy}\xspace}
\newcommand{\treatment}{\ensuremath{\rvt}\xspace}
\newcommand{\covariates}{\ensuremath{\rvx}\xspace}
\newcommand{\latent}{\ensuremath{\rvz}\xspace}
\newcommand{\exogenous}{\ensuremath{\rvu}\xspace}
\newcommand{\covariatei}{\ensuremath{\mathrm{x}}\xspace}
\newcommand{\exogenousi}{\ensuremath{\mathrm{u}}\xspace}

\newcommand{\timepoint}{\ensuremath{\tau}\xspace}
\newcommand{\timevar}{\ensuremath{\taub}\xspace}

\newcommand{\hazard}{\ensuremath{h}\xspace}
\newcommand{\survival}{\ensuremath{S}\xspace}


\newcommand{\samplecov}{\ensuremath{\vx}\xspace}
\newcommand{\samplecovi}{\ensuremath{x}\xspace}
\newcommand{\samplelatent}{\ensuremath{\vz}\xspace}
\newcommand{\samplelatenti}{\ensuremath{z}\xspace}
\newcommand{\sampleoutcome}{\ensuremath{y}\xspace}
\newcommand{\sampleexogenous}{\ensuremath{\vu}\xspace}
\newcommand{\sampleexogenousi}{\ensuremath{u}\xspace}
\newcommand{\sampleparents}[1]{\ensuremath{pa({#1})}\xspace}

% \newcommand{\obssize}{\ensuremath{{D_\rvx}}\xspace}
\newcommand{\covsize}{\ensuremath{{D}}\xspace}
\newcommand{\latentsize}{{\ensuremath{D_\latent}}\xspace}
\newcommand{\samplesize}{\ensuremath{N}\xspace}
\newcommand{\allsize}{\ensuremath{{D_\rvv}}\xspace}
\newcommand{\proxysize}{\ensuremath{{S}}\xspace}

\newcommand{\edges}{\ensuremath{\mathcal{E}}\xspace}
\newcommand{\indexset}{\ensuremath{\mathcal{V}}\xspace}

\newcommand{\leftedge}{L\xspace}
\newcommand{\rightedge}{R\xspace}
\newcommand{\presence}[1]{\textcolor{firstcolor}{#1}}
\newcommand{\absence}[1]{\textcolor{secondcolor}{#1}}

\newcommand{\covspace}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\treatmentspace}{\ensuremath{\mathcal{T}}\xspace}

\newcommand{\splinecoef}{\ensuremath{w_s}\xspace}
\newcommand{\splinebiascoef}{\ensuremath{w_b}\xspace}
\newcommand{\weight}{\ensuremath{\lambda}\xspace}
\newcommand{\samplekan}{\ensuremath{z}\xspace}

% FOR SACHS

\newcommand{\PKC}{\methodname{PKC}\xspace}
\newcommand{\PKA}{\methodname{PKA}\xspace}
\newcommand{\Raf}{\methodname{Raf}\xspace}
\newcommand{\Mek}{\methodname{Mek}\xspace}
\newcommand{\Erk}{\methodname{Erk}\xspace}
\newcommand{\Akt}{\methodname{Akt}\xspace}
\newcommand{\Jnk}{\methodname{Jnk}\xspace}
\newcommand{\Pte}{\methodname{P38}\xspace}
\newcommand{\Plcg}{\methodname{Plcg}\xspace}
\newcommand{\piptwo}{\methodname{PIP2}\xspace}
\newcommand{\pipthree}{\methodname{PIP3}\xspace}

% FOR CARDIO
\newcommand{\age}{\methodname{Age}\xspace}
\newcommand{\obesity}{\methodname{BMI}\xspace}
\newcommand{\diabetes}{\methodname{Diabetes}\xspace}
\newcommand{\hypertension}{\methodname{Systolic pressure}\xspace}
\newcommand{\ischemia}{\methodname{Cardiac ischemia}\xspace}
\newcommand{\mac}{\methodname{MAC event}\xspace}





==> tikz.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LIBRARIES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{
    shapes,
    pgfplots.groupplots,
    shadings,
    calc,
    arrows,
    backgrounds,
    colorbrewer,
    shadows.blur,
    external,
    shapes,
    shapes.arrows,
    shapes.symbols,
    arrows.meta,
    positioning, 
    decorations.pathreplacing,
    intersections,
    cd,
    scopes,
    babel, % otherwise there is an error when importing spanish in babel
    fit % For extending the bounding box
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% STYLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\tikzset{every picture/.style={->, shorten >=1pt, thick}}

% in preamble
\tikzcdset{
    nodes={anchor=center},
    arrow style=tikz,
    diagrams={>={Stealth[scale=0.8]}},
%    diagrams={>={Straight Barb[scale=0.8]}},
}

% \tikzstyle{main node}=[circle,draw,font=\sffamily\Large\bfseries]
\tikzstyle{main node}=[circle,draw,font=\sffamily\small,inner sep=0pt, outer sep=0pt, minimum size=5mm]
\tikzstyle{observed}=[style=main node, fill=gray!25]
\tikzstyle{hidden}=[style=main node, fill=white, dashed, draw=black!40, text=black!60]
\tikzstyle{hiddenarrow}=[dashed, draw=black!40]
\tikzstyle{realobs}=[style=main node,  ellipse]
\tikzstyle{realhidden}=[style=hidden, ellipse]
\tikzstyle{fairnessobs} = [style=main node, ellipse, minimum height=5mm,minimum width=10mm] %Ellipse for fairness
\tikzstyle{fairnesshidden} = [style=main node, ellipse, fill=white, dashed, draw=black!60, text=black!60, minimum height=5mm,minimum width=10mm] %Ellipse for fairness
\tikzset{
    given variable/.style = {
        draw=none, outer sep=0pt, inner sep=0pt, "#1"{yshift=-5pt}
    }
}

\tikzstyle{identifiable}=[draw=idcolor, very thick]
\tikzstyle{nonidentifiable}=[draw=unidcolor, very thick]


\tikzstyle{block} = [rectangle, draw, minimum width=0.5 cm, minimum height=1.5cm]
\tikzstyle{cir} = [circle, draw, minimum size=0.3cm]
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{decision} = [diamond, aspect=2.5, minimum width=3cm, text centered, draw=black]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{hexa} = [trapezium, trapezium left angle=60, trapezium right angle=120, draw,  
      minimum width=2cm, minimum height=0.5cm]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Other commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\irregularcircle[2]{% radius, irregularity
    \pgfextra {\pgfmathsetmacro\len{(#1)+rand*(#2)}}
    +(0:\len pt)
    \foreach \a in {10,20,...,350}{
        \pgfextra {\pgfmathsetmacro\len{(#1)+rand*(#2)}}
        -- +(\a:\len pt)
    } -- cycle
}


\pgfdeclareplotmark{mystar}{
    \node[star,star point ratio=2.25,minimum size=6pt,
    inner sep=0pt,draw=black,solid,fill=red] {};
}


